Use of MESSENGER radioscience data to improve planetary ephemeris and to test general relativity

The current knowledge of Mercury orbit has mainly been gained by direct radar ranging obtained from the 60s to 1998 and by five Mercury flybys made by Mariner 10 in the 70s, and MESSENGER made in 2008 and 2009. On March 18, 2011, MESSENGER became the first spacecraft to orbit Mercury. The radioscience observations acquired during the orbital phase of MESSENGER drastically improved our knowledge of the orbit of Mercury. An accurate MESSENGER orbit is obtained by fitting one-and-half years of tracking data using GINS orbit determination software. The systematic error in the Earth-Mercury geometric positions, also called range bias, obtained from GINS are then used to fit the INPOP dynamical modeling of the planet motions. An improved ephemeris of the planets is then obtained, INPOP13a, and used to perform general relativity tests of PPN-formalism. Our estimations of PPN parameters (beta and gamma?) are more stringent than previous results.

==> messenger-acro.tex <==
%% LaTeX2e file `messenger-acro.tex'
%% generated by the `filecontents' environment
%% from source `messenger' on 2013/06/02.
%%
\renewcommand*{\glstextformat}[1]{\textcolor{black}{#1}}
\newacronym{CNES}{CNES}{Centre National d'Etudes Spatiales}
\newacronym{DSN}{DSN}{Deep Space Network}
\newacronym{ESA}{ESA}{European Space Agency}
\newacronym{GINS}{GINS}{Géodésie par Intégrations Numériques Simultanées}
\newacronym{INPOP}{INPOP}{Intégrateur Numérique Planétaire de l'Observatoire de Paris}
\newacronym{LOS}{LOS}{line of sight}
\newacronym{NAIF}{NAIF}{Navigation and Ancillary Information Facility}
\newacronym{NASA}{NASA}{National Aeronautics and Space Administration}
\newacronym{PDS}{PDS}{Planetary Data System}
\newacronym{SEP}{SEP}{Sun Earth Probe}
\newacronym{VEX}{VEX}{Venus Express}
\newacronym{MGR}{MESSENGER}{MErcury Surface, Space Environment, GEochemistry, and Ranging}
\newacronym{JPL}{JPL}{Jet Propulsion Laboratory}
\newacronym{RMDCT}{RMDCT}{Radio Metric Data Conditioning Team}
\newacronym{ODF}{ODF}{Orbit Data File}
\newacronym{EOP}{EOP}{Earth Orientation Parameters}
\newacronym{IAU}{IAU}{International Astronomical Union}
\newacronym{HEF}{HEF}{mount high efficiency}
\newacronym{BVE}{BVE}{block 5 exciter}
\newacronym{COI}{COI}{center of integration}
\newacronym{PPN}{PPN}{Parametrized Post Newtonian}
\newacronym{ROB}{ROB}{Royal Observatory of Belgium}
\newacronym{rms}{rms}{root mean square}
\newacronym{GR}{GR}{general relativity}

